Distill and De-bias: Mitigating Bias in Face Verification using Knowledge Distillation

Face recognition networks generally demonstrate bias with respect to sensitive attributes like gender, skintone etc. For gender and skintone, we observe that the regions of the face that a network attends to vary by the category of an attribute. This might contribute to bias. Building on this intuition, we propose a novel distillation-based approach called Distill and De-bias (D&D) to enforce a network to attend to similar face regions, irrespective of the attribute category. In D&D, we train a teacher network on images from one category of an attribute; e.g. light skintone. Then distilling information from the teacher, we train a student network on images of the remaining category; e.g., dark skintone. A feature-level distillation loss constrains the student network to generate teacher-like representations. This allows the student network to attend to similar face regions for all attribute categories and enables it to reduce bias. We also propose a second distillation step on top of D&D, called D&D++. Here, we distill the `un-biasedness' of the D&D network into a new student network, the D&D++ network, while training this new network on all attribute categories; e.g., both light and dark skintones. This helps us train a network that is less biased for an attribute, while obtaining higher face verification performance than D&D. We show that D&D++ outperforms existing baselines in reducing gender and skintone bias on the IJB-C dataset, while obtaining higher face verification performance than existing adversarial de-biasing methods. We evaluate the effectiveness of our proposed methods on two state-of-the-art face recognition networks: ArcFace and Crystalface.

==> rough.tex <==
\section*{Supplementary material}
In this supplementary material, we provide the following information:\\
\textbf{Section \ref{supp_sec:relation}}: Relation between face recognition and face verification.\\
\textbf{Section \ref{supp_sec:fairness}}: A novel interpretation of the bias measure (introduced in \cite{Dhar_2021_ICCV}) as a metric for Equality of Odds.\\
\textbf{Section \ref{supp_sec:dndinfo}}: Training details for OSD, D\&D, and D\&D++. \\
\textbf{Section \ref{supp_sec:detailedresult}}: Detailed results with ArcFace (Section \ref{supp_sec:afdetailresult}) and Crystalface (Section \ref{supp_sec:cfdetailresult}) backbones, including verification ROCs. \\
\textbf{Section \ref{supp_sec:passinfo}}: Training details for PASS \cite{Dhar_2021_ICCV} baselines, following the official implementation \cite{passcode}.\\
\textbf{Section \ref{supp_sec:iveinfo}}: Training details for IVE, following the official implementation \cite{ivecode}.\\
\textbf{Section \ref{supp_sec:bowyerinfo}}: Pipeline for obscuring hair (similar to \cite{albiero2020face}). \\
\begin{table}[]
\centering
%\scriptsize
\scalebox{1.0}{
\hskip-0.2cm\begin{tabular}{c|c}
\toprule

    Table/Fig. & Summary  \\
  \midrule
  Table \ref{supp_tab:hpdnd} & Hyperparameters for D\&D,D\&D++,OSD \\
  \midrule
  Fig. \ref{supp_fig:afgstwise}& \thead{Gender \& Skintone-wise verification plots for\\ ArcFace and its debiasing counterparts}\\
  \midrule
  Table \ref{supp_tab:arcstd}& \thead{Tabular values for \textbf{Figure 6} from the main paper}\\
  \midrule
  Fig. \ref{supp_fig:cfwise}& \thead{Gender \& Skintone-wise verification plots for\\ Crystalface and its debiasing counterparts}\\
  \midrule
  Table \ref{supp_tab:cfallbias} & \thead {Gender and skintone bias analysis for Crystyalface-based methods \\ (Extension of \textbf{Table 3} from the main paper)}\\
  \midrule
  Table \ref{supp_tab:crystd}& \thead{Tabular values for \textbf{Figure 7} from the main paper}\\
  \midrule
  Table \ref{supp_tab:hppass} & Hyperparameters for PASS\\
\bottomrule
\end{tabular}
}
\caption{ \textbf{Summary}: For the readers' convenience, we provide a brief summary of the important tables and figures in this supplementary material.} \label{supp_tab:summary}
\end{table}

% \section{Bias measure as metric for Equality of Odds}
\section{Relation between face recognition and face verification}
A face recognition network is trained to classify the identities in a training dataset. Here, we briefly describe the relationship between face recognition and face verification. Any task (such as face veification, identification, authentication etc.) that requires a system to recognize a representation of the input face comes under the umbrella of face recognition.  The most common tasks in the literature \cite{ranjan2019fast,deng2018ArcFace,Swami_2016_triplet} that are used to evaluate a face recognition network are:\\
(i) Face Verification: As defined in \cite{ranjan2019fast}, the aim of this task is to determine if a given pair of templates (i.e. two sets of face representations) belong to the same or different identity. These representations are extracted using previously trained networks. This is also referred to as 1:1 verification.\\
(ii)Face Identification: The aim of this task is to match a probe template to a collection of templates corresponding to many identities; such a collection is referred to as a gallery. This is also referred to as `1:$N$ search'.\\


In the context of mitigating bias, most face recognition networks are evaluated in terms of their face verification performance on different demographic groups, as done in \cite{gong2020jointly,Dhar_2021_ICCV,gac}. Following this, we also evaluate the bias mitigation in face recognition with respect to the face verification task.
\label{supp_sec:relation}
\section{Zero Bias implies Equality of Odds}
\label{supp_sec:fairness}
We use the bias measures introduced in previous bias mitigation work \cite{Dhar_2021_ICCV}. Here, we show that it may be viewed as a measure of \textit{equality of odds} \cite{hardt2016equality} for pair-wise matching in the sense that achieving zero bias (as defined in Eq~\ref{supp_eq:abias}) allows us to achieve equality of odds.

First, we define \text{bias} at a false positive rate (FPR) of $F$ with respect to attribute $A$ as
\begin{equation}
    \text{Bias}^{(F)} = |\text{TPR}^{(F)}_{a_0} - \text{TPR}^{(F)}_{a_1}|,
    \label{supp_eq:abias}
\end{equation}
where $\text{TPR}^{(F)}_{a_*}$ denotes the true positive rate (TPR) on pairs of faces with attribute $A=a_*$ at FPR of $F$.

Next, we show how achieving zero bias in equation~\ref{supp_eq:abias} satisfies equalized odds. First let $\mathcal{F}$ be the set of all face images and let $A : \mathcal{F}\rightarrow \{0, 1\}$ be an indicator on a binary attribute of a face where $0$ corresponds to $a_0$ and $1$ corresponds to $a_1$. Let $\Omega_A \equiv \{(f_1,f_2)\in \mathcal{F}\times\mathcal{F}~|~A(f_1) = A(f_2)\}$ be the set of all pairs of faces with matching attributes and let $Y : \Omega_A \rightarrow \{0,1\}$ indicate identity equivalence for a pair of faces. Since all pairs in $\Omega_A$ consist of faces with equal values of $A$ we extend $A$ onto $\Omega_A$ such that $A(f_1,f_2) = A(f_1)$ for all $(f_1,f_2) \in \Omega_A$. Finally, let $\hat{Y} : \Omega_A \rightarrow \{0,1\}$ be a predictor of $Y$. Supposing $\omega \in \Omega_A$ is random pair of faces sampled from $\Omega_A$, then we have \textit{equality of odds} if and only if
\begin{multline}
    \label{supp_eq:eqoddstpr}
    P(\hat{Y}(\omega)=1|A(\omega)=0,Y(\omega)=1) = \\ P(\hat{Y}(\omega)=1|A(\omega)=1,Y(\omega)=1)
\end{multline}
and
\begin{multline}
    \label{supp_eq:eqoddsfpr}
    P(\hat{Y}(\omega)=1|A(\omega)=0,Y(\omega)=0) = \\ P(\hat{Y}(\omega)=1|A(\omega)=1,Y(\omega)=0).
\end{multline}
Equation~\ref{supp_eq:eqoddstpr} is equivalent to $\text{TPR}^{(F)}_{a_0} = \text{TPR}^{(F)}_{a_1}$ for a fixed FPR of $F$, while equation~\ref{supp_eq:eqoddsfpr} corresponds to a equal FPR for both $a_0$ and $a_1$ pairs.

Equation~\ref{supp_eq:eqoddstpr} is clearly satisfied when the bias measure in equation~\ref{supp_eq:abias} is zero. Equation~\ref{supp_eq:eqoddsfpr} is satisfied by selecting two appropriate thresholds, one for pairs with attribute $A=a_0$ and another for pairs with attribute $A=a_1$. In this way, we have shown that minimizing the bias term defined in equation~\ref{supp_eq:abias} works towards achieving equalized odds in pair-wise face matching.
\section{Training details for D\&D, D\&D++ and OSD}
In this section, we provide hyperparameter and training details for our proposed methods (D\&D and D\&D++) and OSD.
\label{supp_sec:dndinfo}
\begin{table}%
  \centering
\begin{tabular}{ccc}
\toprule
Method/Backbone  & ArcFace & Crystalface\\
\midrule
OSD(g)&$\lambda_{osd}=1.0$&$\lambda_{osd}=0.8$\\
D\&D(g)&$\lambda_1=1.0$& $\lambda_1=1.0$\\
D\&D++(g)&$\lambda_2=1.0$&$\lambda_2=1.0$\\
\midrule
OSD(s)&$\lambda_{osd}=0.5$&$\lambda_{osd}=0.3$\\
D\&D(s)&$\lambda_1=1.0$&$\lambda_1=0.5$\\
D\&D++(s)&$\lambda_2=1.0$&$\lambda_2=0.5$\\
\bottomrule
\vspace{-6pt}
\end{tabular}
\caption{\small  Hyperparameters for training D\&D, D\&D++ and OSD.}
  \label{supp_tab:hpdnd}
\end{table}
\subsection{D\&D and D\&D++}
In Section 4.2 of the main paper, we explain the D\&D and D\&D++ approaches in detail. We define a bias reducing classification loss $L_{br}$ to train the student network $M_s$ in step 2 as
\begin{equation}
    L_{br} = L_{class} + \lambda_1 L_{dis},
\end{equation}
where $\lambda_1$ is used to weight $L_{dis}$ in D\&D. Once $M_s$ is trained, we add another step (step 3) called D\&D++ and initialize a new student network $M^{*}_s$ with $M_s$ and train it on both categories of the binary attribute $A$. During this phase, we constrain $M^{*}_s$ to mimic the teacher $M_s$. So, we train $M^{*}_s$ using the bias reducing classification loss $L_{br}$ defined as
\begin{equation}
    L_{br} = L_{class} + \lambda_2 L_{dis},
\end{equation}
where $\lambda_2$ is used to weight $L_{dis}$ in D\&D++. We list the hyperparameters $\lambda_1$ and $\lambda_2$ in Table \ref{supp_tab:hpdnd}.
\subsection{OSD}
We construct a baseline called One Step Distillation (OSD) by skipping Step 2 of D\&D++. Here, we first train a teacher network $M_t$ that is trained on only one category of attribute $A$ (category $a_{high}$). Then, we initialize a new student network $M^{*}_s$ and train it on both attribute categories of $A$. During this phase, we constrain $M^{*}_{s}$ to mimic $M_t$. To realize this, we feed the given image to both $M^{*}_s$ and $M_t$ and obtain features $f^{*}_s$ and $f_t$, respectively and compute their cosine distance using $L_{dis}$
\begin{equation}
    L_{dis}(f_t,f^{*}_s) =1 - \frac{f_t\cdot f^{*}_s}{\|f_t\|\|f^{*}_s\|}.
\end{equation}
Combining $L_{dis}$ with $L_{class}$, we train $M^{*}_s$ with a bias reducing classification loss $L_{br}$ defined as
\begin{equation}
    L_{br} = L_{class} + \lambda_{osd} L_{dis},
\end{equation}
where $\lambda_{osd}$ is used to weight $L_{dis}$ in OSD.  The difference
between D\&D++ and OSD is that in D\&D++, $M^{*}_s$ uses a teacher ($M_s$) that has information about both of the attribute categories, whereas in OSD, $M^{*}_s$ uses a teacher ($M_s$) with information about only one category.\\


We provide the hyperparameter $\lambda_{osd}$ in Table \ref{supp_tab:hpdnd}. For all the steps in training networks in D\&D, D\&D++ and OSD, we use a batch size of 128. We train the networks for 300 epochs. We start with a learning rate of 0.1 and reduce the learning rate by 10\% after every fifty epochs. We use SGD for optimization.
\section{Detailed results}
\label{supp_sec:detailedresult}
In this section, we provide detailed versions of the results presented in the main paper.
% \begin{figure}
% {
% \centering
% \subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/crystalface_overall_dnd_bupt_latest.pdf}\label{supp_fig:cftpr}}
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_skintone_crystalface_overall_dnd_bupt_skintone_latest.pdf}}
% %\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
% \caption{\small Overall verification plots for IJB-C dataset obtained using Crystalface and its (a) Gender-debiasing, and (b) Skintone debiasing counterparts.}
% \label{supp_fig:cfoverall}
% }
% \end{figure}
% \begin{figure}
% {
% \centering
% \subfloat[Attention maps for male and female faces generated with
% D\&D++(g) are more similar, that those generated with the original Crystalface network.]{\includegraphics[width=\linewidth]{latex/images/qual_res_gender_supp.pdf}\label{supp_fig:qualresupp}}\\
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[Attention maps for faces with dark and light skintone generated with
% D\&D++(s) are more similar, that those generated with the original Crystalface network.]{\includegraphics[width=\linewidth]{latex/images/qual_res_skintone_supp.pdf}}
% %\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
% \caption{\small D\&D++ enforces the networks to attend to similar face regions for both categories of the binary attribute.}
% \label{supp_fig:qualressup}
% }
% \end{figure}
% \begin{figure}
% {
% \centering
% \subfloat[D\&D++(g) (F$\rightarrow$M$\rightarrow$All)]{\includegraphics[width=0.5\linewidth]{latex/images/ijbc_fg2_121000-mm.scores.png}\label{supp_fig:fma}}
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[D\&D++(g) (M$\rightarrow$F$\rightarrow$All)]{\includegraphics[width=0.5\linewidth]{latex/images/ijbc_fg2_51000-mm.scores.png}\label{supp_fig:amf}}\\
% \subfloat[D\&D++(s) (L$\rightarrow$D$\rightarrow$All)]{\includegraphics[width=0.5\linewidth]{latex/images/ijbc_step3_rev_student_142000-light.scores.png}\label{supp_fig:lda}}
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[D\&D++(s) (D$\rightarrow$L$\rightarrow$All)]{\includegraphics[width=0.5\linewidth]{latex/images/ijbc_ds_wt0.2_171000-light.scores.png}\label{supp_fig:dla}}
% %\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
% \caption{\small \textbf{(a,b) }Reversing the sequence in which different genders are learned in Crystalface-based D\&D++(g). Here F=female and M=male subset of BUPT-BalancedFace dataset. \textbf{(c,d)}Reversing the sequence in which different skintones are learned in Crystalface-based D\&D++(s). Here L=light and D=dark subset of BUPT-BalancedFace dataset.}\vspace{-0.5cm}
% \label{supp_fig:genderreverse}
% }
% \end{figure}
% \begin{figure}
% {
% \centering
% \subfloat[]{\includegraphics[width=0.45\linewidth]{latex/images/am_res_gender_v2_reverse.pdf}\label{supp_fig:amgenderrev}}~
% \subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/am_res_skintone_v2_reverse.pdf}\label{supp_fig:amstrev}}
% \vspace{-1em}
% \caption{\small (a.) D\&D++(g) and reverse-ordered D\&D++(g) generate more similar attention maps for male and female frontal faces, as compared to Crystalface. (b.)  D\&D++(s) and reverse-ordered D\&D++(s) generate more similar attention maps for dark and light frontal faces, than Crystalface.}
% %\vspace{-0.7cm}
% \label{supp_fig:avgmapreverse}
% }
% \end{figure}
\subsection{Results with ArcFace}
\label{supp_sec:afdetailresult}
As mentioned in Section 5.3.2 (Table 2) of the main paper, we apply D\&D, D\&D++ and all other de-biasing baselines on the Resnet-50 version of ArcFace \cite{deng2018ArcFace}, and evaluate the gender and skintone bias reduction. In Figure \ref{supp_fig:afgstwise}, we provide the gender-wise and skintone-wise  ROCs for IJB-C, obtained using ArcFace and its debiasing counterparts. In Fig. 6 of the main paper, we also provide the verification plots for all three skintone categories (light, medium, dark) and standard deviation (STD) among these categories, obtained using ArcFace network and its skintone debiasing counterparts. Here, in Table \ref{supp_tab:arcstd}, we present the tabular values of this figure.
\begin{figure}
{
\centering
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/af_gwise.pdf}\label{supp_fig:afgwise}}
%\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/af_stwise.pdf}\label{supp_fig:afstwise}}
%\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
\caption{\small (a) Gender-wise verification plots for ArcFace and its gender-debiasing counterparts. `m-m'=male-male pairs, `f-f'=female-female pairs. For a given method, a \textit{high degree of separation between the male-male curve and female-female curve indicates high gender bias and vice versa}. (b) Skintone-wise verification plots for ArcFace and its skintone-debiasing counterparts. For a given method, \textit{a high degree of separation between the light-light curve and dark-dark curve indicates high skintone bias and vice versa}.}
\label{supp_fig:afgstwise}
}
\end{figure}
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}{c|ccc|ccc|ccc}
 \toprule
 FPR &    & $10^{-4}$   & &  &  $10^{-3}$   &  &  &   $10^{-2}$   &  \\
 \midrule
    Method& TPR\textsubscript{med}& Avg & STD ($\downarrow$)& TPR\textsubscript{med}& Avg & STD ($\downarrow$)&  TPR\textsubscript{med}& Avg & STD ($\downarrow$)\\
  \midrule
ArcFace & 0.883&0.893&0.014&0.921&0.928&0.009&0.954&0.956&0.006\\
IVE(s)$\dag$\cite{terhorst2019suppressing}&0.872&0.956&0.006&0.921&0.928&0.011& 0.964&0.960&0.006\\
PASS-s$\dag$\cite{Dhar_2021_ICCV} & 0.754&0.757&0.016&0.852&0.852&0.005&0.918&0.920&0.002 \\
\midrule
OSD(s) &0.861&0.861&\textbf{0.002}&0.904&0.908&0.007&0.944&0.947&0.004\\
\rowcolor{Gray}
D\&D(s)  & 0.852&0.846&0.007&0.901&0.901&\textbf{0.004}&0.939&0.943&0.003\\
\rowcolor{Gray}
D\&D++(s) & 0.867 & 0.869 & \textbf{0.002}&0.922&0.919&\textbf{0.004}&0.954&0.953&\textbf{0.001} \\
\bottomrule
\end{tabular}
}
\caption{\small Average and Standard deviation (STD) among the verification TPRs of light-light pairs, medium-medium pairs and dark-dark pairs, obtained using ArcFace and its de-biased counterparts. TPR\textsubscript{med}: medium-medium TPR. \textbf{Bold}=Best, \underline{Underlined}=Second best. \textsuperscript{$\dag$}=Our implementation of baselines. All methods are trained on BUPT-BalancedFace \cite{wang2020mitigating} data.}\label{supp_tab:arcstd} \vspace{-0.12cm}
\end{table}
\begin{table}[]
\centering
\scalebox{1.0}{
\begin{tabular}[h]{cccccc}
\hline
 Method/FPR & $10^{-5}$ & $10^{-4}$ & $10^{-3}$  &Training attributes &Training Dataset (\# images)\\ 
\hline
Debface-ID  &0.820 & 0.881&0.895&Race,age,gender&MS-Celeb-1M ($\sim$ 5.8 Million)\\
D\&D++(g)  &0.825&0.880&0.920&Gender&BUPT-BF ($\sim$ 1.2 Million)\\
D\&D++(s) &0.823&0.882&0.926&Race&BUPT-BF($\sim$ 1.2 Million)\\
\bottomrule
\end{tabular}
}
\caption{IJB-C verification performance of ArcFace-based D\&D++ vs. Debface\cite{gong2020jointly}. Debface-ID numbers are obatined from the original paper \cite{gong2020jointly}.}\label{supp_tab:comp}
\label{supp_tab:compsota}
\end{table}
% \begin{figure*}
% {
% \centering
% %\vspace{-0.6cm}
% \subfloat[\scriptsize TPR@FPR=$10^{-5}$ v/s GB (CF)]{\includegraphics[width=0.25\linewidth]{latex/images/cface_gb_1e-5.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-3}$ v/s GB (CF)]{\includegraphics[width=0.25\linewidth]{latex/images/cface_gb_1e-3.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-4}$ v/s STB (CF)]{\includegraphics[width=0.25\linewidth]{latex/images/cfstb_1e-4.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-2}$ v/s STB (CF)]{\includegraphics[width=0.25\linewidth]{latex/images/cfacestb_1e-2.png}}\\
% \subfloat[\scriptsize TPR@FPR=$10^{-5}$ v/s GB (AF)]{\includegraphics[width=0.25\linewidth]{latex/images/aface_gb_1e-5.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-3}$ v/s GB (AF)]{\includegraphics[width=0.25\linewidth]{latex/images/arcface_gb_1e-3.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-4}$ v/s STB (AF)]{\includegraphics[width=0.25\linewidth]{latex/images/arcface_stb_1e-4.png}}
% \subfloat[\scriptsize TPR@FPR=$10^{-2}$ v/s STB (AF)]{\includegraphics[width=0.23\linewidth]{latex/images/arcface_stb_1e-2.png}}
% \caption{TPR at a fixed FPR \textbf{(a,b)} v/s Gender bias(GB) in Crystalface(CF) based models. \textbf{(c,d)} v/s Skintone bias(STB) in CF-based models. \textbf{(e,f)} v/s GB in ArcFace(AF) based models. \textbf{(g,h)} v/s STB in AF-based models.}\label{supp_fig:tradeoffsupp}}

% \end{figure*}

\subsubsection{Comparison with Debface \cite{gong2020jointly}:} In Table 2 of the main paper we compare D\&D++ with other methods including the recently proposed adversarial method PASS \cite{Dhar_2021_ICCV}, and show that D\&D++ consistently obtains higher face verification performance and lower bias than PASS. We note that DebFaceID \cite{gong2020jointly} is another adversarial method proposed for removing protected attributes like gender and race from face representations, that uses a ResNet50 ArcFace backbone (similar to our ArcFace based D\&D++). For the IJB-C dataset, this work reports the overall face verification performance. So, in Table \ref{supp_tab:compsota}, we compare the overall face verification performance obtained by D\&D++ with that obtained by DebfaceID on IJB-C. D\&D++ obtains higher face verication performance than DebfaceID at most FPRs. It should be noted that DebfaceID uses a cleaned version of MS-Celeb-1M (MS1M) dataset \cite{guo2016ms} (provided by \cite{deng2018ArcFace}) for training, which consists of approximately 5.8 million images, whereas  D\&D-based systems are trained on the BUPT-BalancedFace dataset that consists of $\sim$ 1.2 million images. We do not use MS1M dataset as it does not contain race labels. On the other hand, BUPT-BalancedFace \cite{wang2020mitigating} contains race labels, making it easier to train skintone-debiasing models.
% \subsection{Bias v/s face verification performance}
% \label{supp_sec:biasvsperf}
% An ideal de-biasing system must reduce bias and maintain reasonable face verification performance. In Figure 8 of the main paper, we show the TPR at a fixed FPR and gender/skintone bias for several de-biasing methods, including our proposed methods. We fixed the FPR=$10^{-4}$ for gender de-biasing methods, and FPR=$10^{-3}$ for skintone de-biasing methods. Here in Figure \ref{supp_fig:tradeoffsupp}, we provide the same plots for all the other FPRs. In these plots, an ideal de-biasing method would occupy the upper-left-hand corner, where the face verification performance is high, and bias is low, whereas in the worst case scenario, the de-biasing method would occupy the lower left corner which indicates high bias and low face verification performance.
\begin{figure}
{
\centering
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/cf_gwise.pdf}\label{supp_fig:cfgwise}}
%\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/cf_stwise.pdf}\label{supp_fig:cfstwise}}
%\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
\caption{\small (a) Gender-wise verification plots for Crystalface and its gender-debiasing counterparts. `m-m'=male-male pairs, `f-f'=female-female pairs.  For a given method, \textit{a high degree of separation between the male-male curve and female-female curve indicates high gender bias and vice versa}. (b) Skintone-wise verification plots for Crystalface and its skintone-debiasing counterparts. For a given method, \textit{a high degree of separation between the light-light curve and dark-dark curve indicates high skintone bias and vice versa}.}\label{supp_fig:cfwise}
\label{supp_fig:cfgstwise}
}
\end{figure}
\subsection{Results with Crystalface}
\label{supp_sec:cfdetailresult}
For evaluating the generalizability of D\&D, D\&D++ and other baselines, we implement all the methods using the Crystalface \cite{ranjan2019fast} backbone and present the results in Section 5.4 of the main paper. Here, in Tables \ref{supp_tab:cfgenbias},\ref{supp_tab:cfstbias} we extend Tables 3a, 3b (respectively) from the main paper. We also provide the gender-wise and skintone-wise verification ROCs for IJB-C, obtained using all of these methods in Figure \ref{supp_fig:cfgstwise}. In Fig. 7 of the main paper, we also provide the verification plots for all three skintone categories (light, medium, dark) and standard deviation (STD) among these categories, obtained using Crystalface network and its skintone debiasing counterparts. Here, in Table \ref{supp_tab:crystd}, we present the tabular values of this figure.
\begin{table*}[]
\centering
%\scriptsize
\subfloat[Gender bias - Crystalface backbone]{\scalebox{0.73}{
\begin{tabular}{c|ccccc|ccccc|ccccc}
\toprule
 FPR &  &  & $10^{-5}$ &  & &  & &  $10^{-4}$ &  &  &  &  & $10^{-3}$ &  &  \\
 \midrule
  Method & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} \\
 \midrule
Crystalface \hspace{-6pt}&  0.856 &  0.869 & 0.794 & 0.075 & 0 & 0.912 &  0.920 & 0.871 &   0.049 & 0 &  0.950& 0.953& 0.921 & 0.031 & 0 \\
IVE(g)\textsuperscript{$\dag$} \cite{terhorst2019suppressing} & 0.840 & 0.820 & 0.804 & 0.016 & \underline{0.768} & 0.910 & 0.911 & 0.880 & 0.031 & 0.365 & 0.952 & 0.951 & 0.932 & 0.019 & 0.389 \\
W/o hair\textsuperscript{$\dag$} \cite{albiero2020face} & 0.592 & 0.396 & 0.706 & 0.310 & -3.441 & 0.803 & 0.770 & 0.783 & 0.013 & 0.615 & 0.899 & 0.888 & 0.868 & 0.020 & 0.301 \\
PASS-g\textsuperscript{$\dag$} \cite{Dhar_2021_ICCV} &0.691  &0.656 &0.647  &\underline{0.009}  & 0.687& 0.842 &0.832  &0.800  &0.031  &0.291  &0.914  &0.918  &0.890 &0.029  &  0.027 \\
\midrule
OSD(g) & 0.721 & 0.712 & 0.738 & 0.027 & 0.482 & 0.817 & 0.815 & 0.828 & 0.013 & 0.631& 0.895 & 0.888 & 0.908 & 0.020 &0.297  \\
\rowcolor{Gray}
D\&D(g) & 0.705 & 0.693 & 0.706 & 0.013 & 0.650 & 0.805 & 0.805 & 0.813 & \textbf{0.008} & \textbf{0.719} & 0.888 & 0.883 & 0.896 & \underline{0.013} & \underline{0.515} \\
\rowcolor{Gray}
D\&D++(g) & 0.754 & 0.744 & 0.741 & \textbf{0.002} & \textbf{0.854} & 0.844 & 0.841 & 0.830 & \underline{0.011} & \underline{0.701}& 0.914 & 0.910 & 0.907 & \textbf{0.002} & \textbf{0.898}\\
\bottomrule
\end{tabular}
}\label{supp_tab:cfgenbias}}\\
\subfloat[Skintone bias - Crystalface backbone]{\scalebox{0.73}{
\begin{tabular}{c|ccccc|ccccc|ccccc}
 \toprule
 FPR &  &  & $10^{-4}$ &  & &  & &  $10^{-3}$ &  &  &  &  & $10^{-2}$ &  &  \\
 \midrule
    Method & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} \\
  \midrule
Crystalface & 0.912 & 0.906 & 0.867 & 0.038 & 0 &  0.950& 0.945 & 0.925 & 0.020 & 0 & 0.973 & 0.970 & 0.963 & 0.006 & 0 \\
IVE(s)\textsuperscript{$\dag$} \cite{terhorst2019suppressing} & 0.910 & 0.906 & 0.854 & 0.072 &-0.371 &0.950 & 0.948 & 0.909 & 0.038 & -0.900 &0.974  & 0.974 & 0.953 & 0.021 & -2.49 \\
PASS-s\textsuperscript{$\dag$} \cite{Dhar_2021_ICCV} & 0.851 & 0.842& 0.815 & 0.027 & 0.222 & 0.910 & 0.903 &0.886  & 0.016 & 0.158 &0.953  &0.953 & 0.946 & 0.007 & -0.187 \\
\midrule
OSD(s) & 0.848 & 0.819 & 0.841 & 0.022 & 0.351 & 0.916 & 0.899 & 0.913 & 0.015 & 0.214 & 0.961 & 0.953 & 0.959 & 0.006 & -0.012 \\
\rowcolor{Gray}
D\&D(s) & 0.850 & 0.828 & 0.839 & \textbf{0.011} & \textbf{0.643}& 0.916 & 0.903 & 0.904 & \textbf{0.001} & \textbf{0.914} & 0.961 & 0.953 & 0.952 & \textbf{0.001} &\textbf{0.821} \\
\rowcolor{Gray}
D\&D++(s) & 0.886 & 0.875 & 0.862 & \underline{0.013} & \underline{0.629} &  0.934& 0.926 & 0.921 & \underline{0.005} & \underline{0.733} & 0.967 & 0.963 & 0.959 & \underline{0.004} &\underline{0.327}\\
\bottomrule
\end{tabular}}\label{supp_tab:cfstbias}}
\caption{\small Bias analysis for \textit{Crystalface} network, and its de-biased counterparts on IJB-C. TPR: overall True Positive rate, TPR\textsubscript{m}: male-male TPR, TPR\textsubscript{f}: female-female TPR. TPR\textsubscript{l}: light-light TPR, TPR\textsubscript{d}: dark-dark TPR. \textbf{Bold}=Best, \underline{Underlined}=Second best. D\&D variants obtain higher BPC and lower gender bias at most FPRs. \textsuperscript{$\dag$}=Our implementation of baselines (See Sections \ref{supp_sec:passinfo}, \ref{supp_sec:iveinfo}, \ref{supp_sec:bowyerinfo} for details). All methods are trained on BUPT-BalancedFace \cite{wang2020mitigating} data.} \label{supp_tab:cfallbias}
\vspace{-0.2cm}
\end{table*}
\begin{table*}[]
\centering
\scalebox{1.0}{
\begin{tabular}{c|ccc|ccc|ccc}
 \toprule
 FPR   &  & $10^{-4}$   & &  &   $10^{-3}$  &  &  &   $10^{-2}$   &  \\
 \midrule
    Method&  TPR\textsubscript{med} & Avg & STD ($\downarrow$)&  TPR\textsubscript{med}&  Avg & STD ($\downarrow$) & TPR\textsubscript{med}& Avg & STD ($\downarrow$)\\
  \midrule
Crystalface  &0.906  &0.893 & 0.018 &0.939 &0.936  & 0.008  &0.968  &0.967 &  0.003\\
IVE(s)$\dag$\cite{terhorst2019suppressing}   &0.889  &0.883 & 0.022  & 0.941 & 0.933&0.017  &0.967  &0.965  &0.009  \\
PASS-s)$\dag$\cite{Dhar_2021_ICCV}  &0.844 &0.834  &0.013   &0.904   &0.898  &  0.008  &0.946  &0.948  & 0.003 \\
\midrule
OSD(s)  &0.834 & 0.831 &\underline{0.009}  & 0.899 &0.904 &  \underline{0.007}  &0.947  & 0.953 & 0.005 \\
\rowcolor{Gray}
D\&D(s)   &0.829 &0.832  &\textbf{0.005}   &0.889  &0.899 &\underline{0.007}   &0.948  & 0.951&\textbf{0.002} \\
\rowcolor{Gray}
D\&D++(s) & 0.888 &0.875 &0.011  & 0.927 & 0.925 & \textbf{0.003}  &0.963 & 0.962 &\textbf{0.002}\\
\bottomrule
\end{tabular}
}
\caption{\small Average and Standard deviation (STD) among the verification TPRs of light-light pairs, medium-medium pairs and dark-dark pairs, obtained using Crystalface and its de-biased counterparts. TPR\textsubscript{med}: medium-medium TPR. \textbf{Bold}=Best, \underline{Underlined}=Second best. D\&D variants obtain the lowest STD (bias) among the performance of the three skintones. \textsuperscript{$\dag$}=Our implementation of baselines. All methods are trained on BUPT-BalancedFace \cite{wang2020mitigating} data. \vspace{-0.8cm}}\label{supp_tab:crystd}
\end{table*}
% \subsubsection{Results on multiple skintones}
%  A sensitive attribute may have more than two categories. In our context, the skintone attribute consists of three categories: Light, medium, dark. In Eq. 2 of the main paper, we chose to define skintone bias as the difference between the verification TPRs of light-light and dark-dark pairs at a given FPR. Following other works such as \cite{xu2021consistent,wang2020mitigating} we can also define skintone bias as the standard deviation (STD) among the verification TPRs of light-light pairs, medium-medium pairs and dark-dark pairs. In Table \ref{supp_tab:std}, we report these STD values for the D\&D systems (and the corresponding baselines) trained on Crystalface features, along with the average of the TPRs obtained for the three skintone categories. \textit{We find that our proposed D\&D/D\&D++ systems obtain considerably lower STD than existing baselines, thus mitigating skintone bias.} We also provide the skintone-wise verification plots for all three skintones (light, medium and dark) on IJB-C dataset in Figure \ref{supp_fig:lmd}.
% \subsubsection{Reversing the order in D\&D++}
% % \begin{figure}
% % {
% % \centering
% % \subfloat[Crystalface]{\includegraphics[width=0.5\linewidth]{latex/images/cf_lmd.pdf}}
% % \subfloat[IVE(s)]{\includegraphics[width=0.5\linewidth]{latex/images/ive_cf_lmd.pdf}}\\
% % \subfloat[PASS-s]{\includegraphics[width=0.5\linewidth]{latex/images/pass_cf_lmd.pdf}}
% % \subfloat[OSD(s)]{\includegraphics[width=0.5\linewidth]{latex/images/osd_cf_lmd.pdf}}\\
% % \subfloat[D\&D(s)]{\includegraphics[width=0.5\linewidth]{latex/images/dnd_cf_lmd.pdf}}
% % \subfloat[D\&D++(s)]{\includegraphics[width=0.5\linewidth]{latex/images/dnd++_cf_lmd.pdf}}
% % \caption{\small Skintone-wise verification ROCs for all three skintones (light, medium, dark) in IJB-C for Crystalface and its de-biasing counterparts. }
% % \label{supp_fig:lmd}
% % }
% % \end{figure}
% In Section 5.4.3 (Table 4) of the main paper we discuss the effect of reversing the order in which different genders are learned in D\&D++(g). We provide the detailed results for this experiment in Table \ref{supp_tab:reverse} (top row). The gender-wise verification plots on IJB-C dataset for both D\&D++(g) trained with sequence Female(F)$\rightarrow$Male(M)$\rightarrow$All and that with sequence Male(M)$\rightarrow$Female(F)$\rightarrow$All are provided in Figures \ref{supp_fig:fma} and \ref{supp_fig:amf} respectively. We perform the same experiment with respect to the skintone attribute by reversing the order in which different skintones are learned in D\&D++(s) and present the results in Table \ref{supp_tab:reverse} (bottom row). The skintone-wise verification plots on IJB-C dataset for both D\&D++(s) trained with sequence Light(L)$\rightarrow$Dark(D)$\rightarrow$All and that with sequence Dark(D)$\rightarrow$Light(L)$\rightarrow$All are provided in Figure \ref{supp_fig:lda} and \ref{supp_fig:dla} respectively. Additionally, in Fig. \ref{supp_fig:avgmapreverse}, we also provide the average attention maps for frontal male and female faces (generated by D\&D++(g) and reverse-ordered D\&D++(g)), and for frontal faces with light and dark skintone (generated by D\&D++(s) and reverse-ordered D\&D++(s)).
% \begin{table*}[]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{c|ccccc|ccccc|ccccc}
%  \toprule
%  FPR &  &  & $10^{-4}$ &  & &  & &  $10^{-3}$ &  &  &  &  & $10^{-2}$ &  &  \\
%  \midrule
%     Method& TPR\textsubscript{l} & TPR\textsubscript{med}& TPR\textsubscript{d}& Avg & STD ($\downarrow$)& TPR\textsubscript{l} & TPR\textsubscript{med}& TPR\textsubscript{d}& Avg & STD ($\downarrow$)& TPR\textsubscript{l} & TPR\textsubscript{med}& TPR\textsubscript{d}& Avg & STD ($\downarrow$)\\
%   \midrule
% Crystalface & 0.906 &0.906 & 0.867 &0.893 & 0.018 & 0.945&0.939 & 0.925 &0.936  & 0.008 &  0.970 &0.968 & 0.963 &0.967 &  0.003\\
% IVE(s)$\dag$\cite{terhorst2019suppressing}  & 0.906 &0.889 & 0.854 &0.883 & 0.022 & 0.948 & 0.941& 0.909 & 0.933&0.017    & 0.974 &0.967 & 0.953 &0.965  &0.009  \\
% PASS-s)$\dag$\cite{Dhar_2021_ICCV} & 0.842 &0.844 & 0.815 &0.834  &0.013  & 0.903 &0.904 &0.886  &0.898  &  0.008 &0.953 &0.946 & 0.946 &0.948  & 0.003 \\
% \midrule
% OSD(s)  & 0. 819 &0.834 & 0.841& 0.831 &\underline{0.009}  & 0.899 & 0.899& 0.913 &0.904 &  \underline{0.007} & 0.953 &0.947 & 0.959 & 0.953 & 0.005 \\
% \rowcolor{Gray}
% D\&D(s)  & 0.828 &0.829 & 0.839 &0.832  &\textbf{0.005}  & 0.903 &0.889 & 0.904 &0.899 &\underline{0.007}  & 0.953 &0.948 & 0.952 & 0.951&\textbf{0.002} \\
% \rowcolor{Gray}
% D\&D++(s) & 0.875 & 0.888& 0.862 &0.875 &0.011  & 0.926 &0.927 & 0.921 & 0.925 & \textbf{0.003}  & 0.963 &0.963 & 0.959 &0.962 &\textbf{0.002}\\
% \bottomrule
% \end{tabular}
% }
% \caption{\small Average and Standard deviation (STD) among the verification TPRs of light-light pairs, medium-medium pairs and dark-dark pairs. TPR: overall True Positive rate, TPR\textsubscript{l}: light-light TPR, TPR\textsubscript{med}: medium-medium TPR, TPR\textsubscript{d}: dark-dark TPR. \textbf{Bold}=Best, \underline{Underlined}=Second best. D\&D variants obtain the lowest STD (bias) among the performance of the three skintones. \textsuperscript{$\dag$}=Our implementation of baselines (See Sections \ref{supp_sec:passinfo}, \ref{supp_sec:iveinfo}, \ref{supp_sec:bowyerinfo} for details). All methods are trained on BUPT-BalancedFace \cite{wang2020mitigating} data.}\label{supp_tab:std} \vspace{-0.12cm}
% \end{table*}
% \begin{table*}[]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{c|ccccc|ccccc|ccccc}
% \toprule
%  FPR &  &  & $10^{-5}$ &  & &  & &  $10^{-4}$ &  &  &  &  & $10^{-3}$ &  &  \\
%  \midrule
%   Sequence & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{m} & TPR\textsubscript{f} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{g}$(\uparrow)$ \hspace{-4pt} \\

% F$\rightarrow$M$\rightarrow$All & 0.754 & 0.744 & 0.741 & 0.002 & \textbf{0.854} & 0.844 & 0.841 & 0.830 & 0.011 & 0.701& 0.914 & 0.910 & 0.907 & 0.002 & 0.898\\
% M$\rightarrow$F$\rightarrow$All&0.703 & 0.711 & 0.735 & 0.024 & 0.501  &  0.813& 0.821 & 0.817 & 0.004 & \textbf{0.809} & 0.893 & 0.897 & 0.897 & 0 & \textbf{0.940}\\
% \midrule
% FPR &  &  & $10^{-4}$ &  & &  & &  $10^{-3}$ &  &  &  &  & $10^{-2}$ &  &  \\
%  \midrule
%   Sequence & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} \\

% L$\rightarrow$D$\rightarrow$All & 0.886 & 0.875 & 0.862 & 0.013 & \textbf{0.629} &  0.934& 0.926 & 0.921 & 0.005 & \textbf{0.733} & 0.967 & 0.963 & 0.959 & 0.004 &\textbf{0.327 }\\
% D$\rightarrow$L$\rightarrow$All& 0.849 & 0.839 & 0.827 & 0.012 &0.615 &0.913&0.908&0.897&0.010&0.461&0.951&0.956&0.950&0.006&-0.023\\
% \bottomrule
% \end{tabular}
% }
% \caption{\small Reversing the order in which different genders/skintones are learned in (top) D\&D++(g) and (bottom) D\&D++(s). Here, L=light and D=dark skintone subset of BUPTBalancedFace. Similarly, F=female and M=male subset of the dataset. `All' refers to the entire dataset, required for trainng step 3 of D\&D++.}\label{supp_tab:reverse} \vspace{-0.12cm}
% \end{table*}
% \begin{table*}[]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{c|ccccc|ccccc|ccccc}
% \toprule
%  FPR &  & {  } & {  $10^{-4}$} & {  } & {  } & {  } & {  } & {  $10^{-3}$} & {  } & {  } & {  } & {  } & {  $10^{-2}$} & {  } & {  } \\
%  \midrule
%   Method & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} & TPR & TPR\textsubscript{l} & TPR\textsubscript{d} & Bias$(\downarrow)$ \hspace{-4pt} & \hspace{-4pt} BPC\textsubscript{st}$(\uparrow)$ \hspace{-4pt} \\
%   \midrule
% ArcFace & 0.914 & 0.912 & 0.883 & 0.029 & 0 & 0.944 &0.942 & 0.922
%  & 0.021 & 0 & 0.964 & 0.964 & 0.950 & 0.014 & 0 \\
% IVE(s))$\dag$\cite{terhorst2019suppressing} &0.913& 0.911 & 0.871 & 0.040 & -0.380 & 0.943 & 0.941 & 0.919 & 0.022
%  & -0.049 & 0.964 & 0.962 & 0.951 & 0.011 &  0.214\\
% PASS-s)$\dag$\cite{Dhar_2021_ICCV} & 0.786& 0.778 & 0.738 & 0.041 &-0.554 & 0.861 & 0.859 & 0.846 & 0.014 & 0.245 & 0.920 &0.921 &0.922  & \textbf{0.001} & \textbf{0.883} \\
%  \midrule
% OSD(s) & 0.877 &0.864  & 0.859 & \underline{0.005} & \underline{0.787} & 0.923 & 0.918 & 0.901 & 0.016 & 0.216 & 0.956 & 0.953 & 0.944 & 0.009 & 0.349 \\
% \rowcolor{Gray}
% D\&D(s) & 0.855 & 0.836 & 0.851 & 0.015 & 0.418 & 0.913 & 0.906 & 0.895 & \textbf{0.011} & \underline{0.443} & 0.951 & 0.947 & 0.942 & 0.005 & 0.629\\
% \rowcolor{Gray}
% D\&D++(s) & 0.882 & 0.871 & 0.868 & \textbf{0.003} & \textbf{0.862} & 0.926 & 0.923 & 0.912 & \textbf{0.011} &  \textbf{0.457}& 0.957 & 0.954 & 0.951 & \underline{0.003} & \underline{0.778}\\
% \bottomrule
% \end{tabular}
% }
% \caption{\small \textit{Skintone} bias analysis for \textit{ArcFace} network, and its de-biased counterparts on IJB-C. TPR: overall True Positive rate, TPR\textsubscript{l}: light-light TPR, TPR\textsubscript{d}: dark-dark TPR. \textbf{Bold}=Best, \underline{Underlined}=Second best. D\&D variants obtain higher BPC\textsubscript{st} and lower skintone bias at most FPRs. \textsuperscript{$\dag$}=Our implementation of baselines (See Sections \ref{supp_sec:passinfo}, \ref{supp_sec:iveinfo}, \ref{supp_sec:bowyerinfo} for details). All methods are trained on BUPT-BalancedFace \cite{wang2020mitigating} data.}\label{supp_tab:afstbias} \vspace{-0.12cm}
% \end{table*}
% \begin{figure}
% {
% \centering
% \subfloat[Attention maps for male and female faces generated with
% D\&D++(g) are more similar, that those generated with the original ArcFace network.]{\includegraphics[width=\linewidth]{latex/images/qual_res_gender_supp_arcface.pdf}\label{supp_fig:afgenqualres}}\\
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[Attention maps for faces with dark and light skintone generated with
% D\&D++(s) are more similar, that those generated with the original ArcFace network.]{\includegraphics[width=\linewidth]{latex/images/qual_res_skintone_supp_arcface.pdf}\label{supp_fig:afstqualres}}
% %\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_cf_skintone_bupt_dnd_barplot_all6_new.pdf}}
% \caption{\small D\&D++ enforces the networks to attend to similar face regions for both categories of the binary attribute.}
% \label{supp_fig:afqualres}
% }
% \end{figure}
% \begin{figure}
% {
% \centering
% \subfloat[]{\includegraphics[width=0.5\linewidth]{images/arcface_50_gender_bupt.pdf}\label{supp_fig:aftpr}}
% %\subfloat[Gender bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_af_gender_bupt_dnd_barplot_all7.pdf}}
% \subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_skintone_arcface_overall_dnd_bupt_skintone_latest.pdf}}
% %\subfloat[Skintone bias plots]{\includegraphics[width=0.5\linewidth]{latex/images/aaai_af_skintone_bupt_dnd_barplot_all6_new.pdf}}
% \caption{\small Overall verification plots for IJB-C dataset obtained using ArcFace and its (a) Gender-debiasing, and (b) Skintone debiasing counterparts}
% \label{supp_fig:afoverall}
% }
% \end{figure}
\section{Training details for PASS \cite{Dhar_2021_ICCV}}
\label{supp_sec:passinfo}
\subsection{Brief summary of PASS}
PASS \cite{Dhar_2021_ICCV} is composed of three components:\\
(1) \textbf{Generator model $M$}: A model that accepts face recognition feature $f_{in}$ from a pre-trained network, and generates a lower dimensional feature $f_{out}$ that is supposed to be agnostic to sensitive attribute (gender or skintone). $M$ consists of a single linear layer, followed by a PReLU \cite{he2015deep} layer. \\
(2) \textbf{Classifier} $C$: A classifier that takes in $f_{out}$ and generates a prediction vector for identity classification.\\
(3) \textbf{Ensemble of attribute classifiers $E$}: An ensemble of $K$ attribute prediction models. Each of these models is a two layer MLP with 128 and 64  hidden units respectively with SELU activations, followed by a sigmoid activated output layer with $N_{att}$ units,  where $N_{att}$ = the number of classes in the attribute being considered.

 We use the official implementation of PASS \cite{passcode} to build PASS-g (for reducing gender information in face recognition feature) and PASS-s (for reducing skintone information). We provide a brief summary of PASS training, and specify the hyperparameters used. More details are provided on the original paper \cite{Dhar_2021_ICCV} \\
\textbf{Stage 1 - Initializing and training $M$ and $C$}: Using input features $f_{in}$ from a pre-trained network, we train $M$ and $C$ from scratch for $T_{fc}$ iterations using $L_{class}$. $L_{class}$ is a the standard cross entropy classification loss. The learning rate used to train $M$ and $C$ in this stage is denoted by $\alpha_1$. \\
\textbf{Stage 2 - Initializing and training $E$}: Once $M$ is trained to perform classification, we feed the outputs $f_{out}$ of $M$ to ensemble $E$ of $K$ attribute prediction models. $E$ is then trained to classify attribute for $T_{atrain}$ iterations using $L_{att}$. $L_{att}$ is a cross-entropy classification loss for classifying attributes. The learning rate used to train the models in $E$ in this stage is denoted by $\alpha_2$. Model $M$ remains frozen in this step.\\ 
\textbf{Stage 3 - Update model $M$ and classifier $C$}: Here, $M$ is trained to generate features $f_{out}$ that can classify identities and have reduced encoding of  sensitive attribute under consideration. We feed $f_{out}$ to $E$ and $C$, the outputs of which result in an adversarial de-biasing loss $L_{deb}$ and $L_{class}$ respectively. We combine them to compute the bias reducing classification loss in PASS denoted as $L^{(PASS)}_{br}$
\begin{equation}
    L^{(PASS)}_{br} = L_{class} + \lambda L_{deb},
\end{equation}
$L^{(PASS)}_{br}$ is used for training $M$ and $C$ for $T_{deb}$ iterations, while $E$ remains locked. $\lambda$ is used to weight the adversarial loss $L_{deb}$. The learning rate used to train $M$ and $C$ in this stage is denoted by $\alpha_3$.\\
\textbf{Stage 4 - Update ensemble $E$ (discriminator)}:
% In stage 3, $M$ is trained to generate attribute-debiased descriptors $f_{out}$ to fool the models in $E$, whereas in stage 4
In stage 4, members of $E$ are trained to classify attribute using $f_{out}$. So, stages 3 and 4 are run alternatively, for $T_{ep}$ episodes, after which all the models in $E$ are re-initialized and re-trained (as done in stage 2). Here, one episode indicates an instance of running stages 3 and 4 consecutively. In stage 4, following the discriminator-training strategy introduced by \cite{Dhar_2021_ICCV}, we choose one of the models in $E$, and train it for $T_{plat}$ iterations or until it reaches an accuracy of $A^*$ on the validation set. $M$ and $C$ remain frozen in this stage.
\begin{table}%
  \small
  \centering
\begin{tabular}{cccc|cc}
\toprule
Backbone  & &\multicolumn{2}{c|}{ArcFace} & \multicolumn{2}{c}{Crystalface}\\
\midrule
Hyperparam & Stage & PASS-g & PASS-s& PASS-g & PASS-s \\
\midrule
$\lambda$ & 3&10&10&1&10\\
$K$ & 2, 3, 4 &3&2&4&2\\
$T_{fc}$ & 1  &10000&10000&16000&16000\\
$T_{deb}$ & 3 &1200&1200&1200&1200\\
$T_{atrain}$ & 2 &30000&30000&30000&30000\\
$T_{plat}$ & 4  &2000&2000&2000&2000\\
$A^*$ &  4&0.95&0.95&0.90&0.95\\
$\alpha_1$ & 1 &$10^{-2}$&$10^{-2}$&$10^{-2}$&$10^{-2}$\\
$\alpha_2$ &  2,4&$10^{-3}$&$10^{-3}$&$10^{-3}$&$10^{-3}$\\
$\alpha_3$ &  3&$10^{-4}$&$10^{-4}$&$10^{-4}$&$10^{-4}$\\
$T_{ep}$ & 3,4 &40&40&40&40\\
\bottomrule
\vspace{-6pt}
\end{tabular}
\caption{\small  Hyperparameters for training PASS-g and PASS-s on ArcFace and Crystalface features}
  \label{supp_tab:hppass}
  \vspace{-11pt}
\end{table}
\subsection{Datasets and Hyperparameters for PASS}
In the original paper \cite{Dhar_2021_ICCV}, $f_{in}$ is obtained from a pre-trained ArcFace network that has been trained on the MS1MV2 \cite{ms1mv2} dataset. We note that the authors of PASS \cite{Dhar_2021_ICCV} perform experiments using the ResNet 101 version of the ArcFace network. But, in our preliminary experiments, we found that the ResNet50 version of ArcFace network demonstrates more gender and skintone bias, as shown in Figures \ref{supp_fig:50vs100} and \ref{supp_fig:50vs100bias}. With this reasoning, and following some other previous works \cite{gong2020jointly,gac}, we use the Resnet 50 version of ArcFace in our experiments, which is unlike the experiments in PASS\cite{Dhar_2021_ICCV}.


Also, in the original PASS \cite{Dhar_2021_ICCV} paper, PASS-g is trained on a mixture of UMDFaces\cite{bansal2017umdfaces}, UMDFaces-Videos\cite{bansal2017s} and MS1M \cite{guo2016ms}. However, due to the current unavailability of the UMDFaces and UMDFaces-Videos dataset and to make PASS variants comparable with D\&D (and OSD) variants,  we obtain $f_{in}$ from a ArcFace network that has been trained on the BUPT-BalancedFace \cite{wang2020mitigating}, following which we train both PASS-g and PASS-s using the BUPT-BalancedFace dataset as well.  

We note that the authors of PASS\cite{Dhar_2021_ICCV} also perform experiments on Crystalface \cite{ranjan2019fast} trained on the aforementioned  `mixture' dataset. Due to the current unavailability of this dataset, in our implementation, we extract $f_{in}$ using a pre-trained Crystalface network trained on BUPT-BalancedFace dataset. Following that, we train both PASS-g and PASS-s using the BUPT-BalancedFace dataset as well.


We use the same hyperparameters specified in the original paper \cite{Dhar_2021_ICCV} and present them in Table \ref{supp_tab:hppass}.  We use a batch size of 400 in all these experiments. In our work, we use the official implementation of PASS \cite{passcode}.
\begin{figure}
{
\centering
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/gender_arcface_50_vs_100.pdf}\label{supp_fig:gen50vs100}}~
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/st_arcface_50_vs_100.pdf}\label{supp_fig:st50vs100}}
\vspace{-1em}
\caption{\small (a) Gender-wise and (b) Skintone-wise verification ROCs on the IJB-C dataset, for Resnet50 and Resnet101 version of the ArcFace networks, trained on BUPT-BalancedFace dataset. }
%\vspace{-0.7cm}
\label{supp_fig:50vs100}
}
\end{figure}
\begin{figure}
{
\centering
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/gender_barplot_arcface_50vs100.pdf}\label{supp_fig:gen50vs100bar}}~
\subfloat[]{\includegraphics[width=0.5\linewidth]{latex/images/st_barplot_arcface_50vs100.pdf}\label{supp_fig:st50vs100bar}}
\vspace{-1em}
\caption{\small (a) Gender bias and (b) Skintone bias on the IJB-C dataset, for Resnet50 and Resnet101 version of the ArcFace networks, trained on BUPT-BalancedFace dataset. }
%\vspace{-0.7cm}
\label{supp_fig:50vs100bias}
}
\end{figure}
\section{Training details for IVE \cite{terhorst2019suppressing}}
\label{supp_sec:iveinfo}
IVE \cite{terhorst2019suppressing} is an attribute suppression algorithm that assigns a score to each variable in face representations using a decision tree ensemble. This score of a variable indicates the importance of that variable for a specific recognition task. Variables that affect attribute classification considerably are then excluded from the representation. In every exclusion step, $n_e$ variables are removed from the representation. The algorithm is run for $n_s$ steps, thus resulting in exclusion of $n_s \times n_e$ variables from the representation. We follow the re-implementation of IVE by \cite{Dhar_2021_ICCV} and construct two variants of IVE: IVE(g) for reducing gender information and IVE(s) for reducing skintone information. \\

IVE is a feature-based system that reduces information of sensitive attribute from features obtained using a pre-trained network (like ArcFace or Crystalface). So before training IVE, we first train a Resnet 50 version of the ArcFace network on the BUPT-BalancedFace dataset. After that, we train IVE(g) and IVE(s) (separately) as follows:\\
\textbf{Training IVE(g)} : We extract ArcFace features for the images in BUPT-BalancedFace dataset. We also obtain the gender labels for these images using \cite{ranjan2017all}. Then we use the IVE system (explained in \cite{terhorst2019suppressing}) to remove variables in the features that encode gender information. During inference, we use the trained IVE(g) system to transform the ArcFace features extracted for the evaluation dataset (IJB-C).\\
\textbf{Training IVE(s)}: We follow the same experimental setup for training IVE(s). The only difference is that in IVE(s), instead of gender labels, we feed the race label (already provided in the BUPT-BalancedFace dataset) alongwith the ArcFace features extracted for the images in BUPT-BalancedFace dataset. For inference, we use the trained IVE(s) system to transform ArcFace features for IJB-C.\\ 

We perform the same experiment by replacing the pre-trained ArcFace network with a Crystalface network trained on BUPT-BalancedFace dataset, for our Crystalface-based experiments. The official implementation for training IVE is publicly available \cite{ivecode}. In all of our IVE experiments, we use the parameters values mentioned in the code, i.e. $n_s=20$ and $n_e=5$, thus resulting in 100 eliminations. Since face recognition features from ArcFace or Crystalface are 512-dimensional, the trained IVE(s/g) framework transforms the input features for test images into 412 dimensional features, which are then used to perform face verification.
\begin{figure}
\centering
{\includegraphics[width=\linewidth]{latex/images/baseline_bowyer_dnd.pdf}}
%\vspace{-1em}
\caption{\small Our method for obscuring hair (Similar to \cite{albiero2020face}). On the right, we show an aligned image without obscuring hair.}
\label{supp_fig:bowyerbaseline}
\vspace{-6pt}
\end{figure}
\section{Pipeline for obscuring hair}
\label{supp_sec:bowyerinfo}
In \cite{albiero2020face}, the authors obscure hair regions of images in the evaluation dataset. This is done to get an equal fraction of pixels in the images for each gender. The authors use a segmentation network \cite{yu2018bisenet} to obscure the hair.  As a result of obscuring hair, it is shown that the resulting face recognition features extracted using ArcFace demonstrate lower gender bias.  However, as pointed out by \cite{Dhar_2021_ICCV}, such experiments are only performed on datasets with clean frontal faces in MORPH \cite{ricanek2006morph} and Notre-Dame \cite{phillips2005overview} datasets.  But, complex datasets like IJB-C contain varied and cluttered poses, which is why segmentation cannot be used (especially for images with extreme poses). So, following \cite{Dhar_2021_ICCV}, we compute the face border keypoints using \cite{ranjan2017all} and obscure all the regions outside the polygon formed by these keypoints. Our hair obscuring pipeline is presented in Fig \ref{supp_fig:bowyerbaseline}. Note that, this baseline method cannot be used for mitigating skintone bias. After obscuring hair regions for images in the IJB-C dataset, we extract their features using pre-trained Crystalface/ArcFace networks trained on BUPT-BalancedFace, and perform 1:1 face verification.
